Denoising after Entropy-based Debiasing A Robust Training Method for Dataset Bias with Noisy Labels

Improperly constructed datasets can result in inaccurate inferences. For instance, models trained on biased datasets perform poorly in terms of generalization (i.e., dataset bias). Recent debiasing techniques have successfully achieved generalization performance by underestimating easy-to-learn samples (i.e., bias-aligned samples) and highlighting difficult-to-learn samples (i.e., bias-conflicting samples). However, these techniques may fail owing to noisy labels, because the trained model recognizes noisy labels as difficult-to-learn and thus highlights them. In this study, we find that earlier approaches that used the provided labels to quantify difficulty could be affected by the small proportion of noisy labels. Furthermore, we find that running denoising algorithms before debiasing is ineffective because denoising algorithms reduce the impact of difficult-to-learn samples, including valuable bias-conflicting samples. Therefore, we propose an approach called denoising after entropy-based debiasing, i.e., DENEB, which has three main stages. (1) The prejudice model is trained by emphasizing (bias-aligned, clean) samples, which are selected using a Gaussian Mixture Model. (2) Using the per-sample entropy from the output of the prejudice model, the sampling probability of each sample that is proportional to the entropy is computed. (3) The final model is trained using existing denoising algorithms with the mini-batches constructed by following the computed sampling probability. Compared to existing debiasing and denoising algorithms, our method achieves better debiasing performance on multiple benchmarks.

==> main/method_bak.tex <==
\section{\underline{DEN}oising after \underline{E}ntropy-based De\underline{B}iasing}
\label{sec:method}


% \begin{wrapfigure}[17]{r}{0.5\textwidth}
% \vspace{-0.2in}
    % \begin{minipage}[t]{0.5\textwidth}
    % \begin{algorithm}[!t]
    \begin{algorithm}[!t]
    \DontPrintSemicolon
    \SetAlgoLined
    \SetNoFillComment
    \LinesNotNumbered 
    \caption{Deneb: \underline{Den}oising after \underline{e}ntropy-based de\underline{b}iasing}
    \label{alg:deneb}
        \KwInput{Training set $\mc{D}$, Denoising algorithm $\mc{A}_\text{den}$, Epoch $E$, GCE parameter $q$, Temperature parameter $\tau$.}
        \KwOutput{Debiased model.}
        
        % \code{/*  Train biased model */}\\
        \While{$e < E$\tcp*{Train prejudice model $f_p$}} 
        {   
            Update $f_b$ by $\mc{L}_{\text{GCE}}(x,y)$ \tcp*{Eq.~(\ref{eq:gce})} 
            Compute entropy $\mc{H}_e(x,\tau)$ \tcp*{Eq.~(\ref{eq:weight})}
        }
        % \code{/*  Compute score */}\\
        % Compute score $\mc{E}(x)$ \tcp*{Eq.~(\ref{eq:ent_margin})} 
        % \code{/*  Denoising */}\\
        \While{$e < E$\tcp*{Train ultimate model $f_u$}} 
        {   
            Batch sampling with $\mc{P}(x)$ \tcp*{Eq.~(\ref{eq:sampling_prob})} 
            Denoising on batch $\mc{A}_{\text{den}} (B)$
        }
    
    \end{algorithm}
% \end{minipage}
% \end{wrapfigure}

In this section, we introduce \alg, a robust training algorithm for DBwNL. \alg~is highly motivated from the findings in Section~\ref{sec:debiasing},~\ref{sec:denoising}. (1) Entropy (\ie label-free metric) is essential for the DBwNL data set. (2) Denoising should be performed after bias-conflicting samples become confident regardless of label corruption. Figure~\ref{fig:alg} illustrates a brief overview. \alg~composed of two architecture set: (1) prejudiced model, and (2) ultimate model. At each epoch $e$, the prejudice model $f_p$ is trained on the given training dataset $\mc{D}$ and accumulates the entropy score per sample $\mc{W}_e(x)$. After training the prejudice model, calculate the weights for each sample to mitigate dataset bias. Finally, train the ultimate model $f_u$ based on the reconstructed mini-batches of weight training $\mc{E}(x)$. The mini-batches over-samples bias-conflicting and under-samples bias-aligned samples, respectively. Algorithm~\ref{alg:deneb} describe the full steps.


% \alg~composed of three different networks, biased $f_b$, debiased-1 $f_d^1$, and debiased-2 $f_d^2$. At each epoch, the biased model is trained on the given training dataset $\mc{D}$, and reconstruct $\widehat{\mc{D}}$ so that the portion of bias-conflicting samples increases for debiased models. From the dataset sufficiently balanced by the biased model, both debiased models are able to erase noisy labels using \code{f-dividemix}~\cite{kim2021fine}, complementarily. Hereinafter, all methods are described in $f_d^1$ point of view, but it can be straightforwardly applied to $f_d^2$. Algorithm~\ref{alg:deneb} describe the full steps. 


\begin{figure}[t!]
    \centering
    \includegraphics[width=1.0\linewidth]{fig/deneb.pdf}
    \caption{\alg~sequentially trains two networks: prejudice, and ultimate. At each epoch, the prejudiced model is trained with generalized cross entropy loss (GCE) and accumulate entropy of each samples. Sampling probability $\mc{P}(x)$ is computed to be proportional to the average accumulated entropy. The ultimate network is trained on the batches sampled with probability $\mc{P}(x)$. Any denoising algorithms are applicable for denoising phase.}
    \label{fig:alg}
\end{figure}



% In this section, we introduce \alg, a debiasing algorithm when the noisy labels are in the given training dataset. Brief overview is shown in Figure~\ref{fig:alg}. \alg composed of three different networks, biased $f_b$, debiasing-1 $f_{d}^1$, debiasing-2 $f_{d}^2$. At each epoch, the biased model trained on the given noisy biased dataset. Simultaneously, the debiasing models perform co-dividing which split the training dataset into the regarded as clean labeled $\mc{D}_L$, and remains unlabeled $\mc{D}_U$ subsets. Each debiasing model is trained with two types: (1) conventional feed-forward based learning for $\mc{D}_L$ set, (2) co-refinement and co-guessing between two denoising models based on \code{MixMatch}. Algorithm~\ref{alg:deneb} describe the full steps in detail.

% \begin{figure}[h!]
%     \centering
%     \subfloat[$\alpha = 5\%$, $\eta = 10\%$]
%     {\label{fig:stats_5_10}\includegraphics[width=0.225\linewidth]{example-image}}
%     \hspace{0.1in}
%     \subfloat[$\alpha = 5\%$, $\eta = 85\%$]
%     {\label{fig:stats_5_85}\includegraphics[width=0.225\linewidth]{example-image}}
%     \hspace{0.1in}
%     \subfloat[$\alpha = 1\%$, $\eta = 10\%$]
%     {\label{fig:stats_1_10}\includegraphics[width=0.225\linewidth]{example-image}}
%     \hspace{0.1in}
%     \subfloat[$\alpha = 1\%$, $\eta = 85\%$]
%     {\label{fig:stats_1_85}\includegraphics[width=0.225\linewidth]{example-image}}
%     \caption{Statistics of biased dataset with noisy labels. $\alpha$ and $\eta$ represent bias ratio and noisy ratio, respectively.}
%     \label{fig:statistics}
% \end{figure}


\subsection{Robust training for the DBwNL dataset} 


\myparagraph{Training the biased model.} 
Similar to the previous strategy~\cite{nam2020learning,lee2021learning}, we use generalized cross-entropy (GCE)~\cite{zhang2018generalized} to train the biased models. The GCE loss $\mc{L}_{\text{GCE}}$ is indicated as follows:
\begin{equation}
\label{eq:gce}
    \mc{L}_{\text{GCE}}(x,y,\tau) = \frac{1-f(x,\tau)[y]^q}{q},
\end{equation}
where $f(x,\tau)[j]$ denotes the softmax output of the model $f$ with temperature $\tau$ for class $j$, \ie $f(x,\tau)[j] = \frac{\exp (g(x)[j]/\tau)}{\sum_c \exp (g(x)[c]/\tau)}$ with logit $g(x)$. This loss function can be interpreted as a standard cross-entropy loss when $q \to 0$ and as a MAE / unhindered loss when $q=1$. $\mc{L}_{\text{GCE}}$ emphasizes the sample that shows strong agreement between the softmax output and the given label. In other words, it prioritizes samples that are easy-to-learn, such as \code{(Clean, Bias-aligned)} samples.



\myparagraph{Computing entropy-based weight.}
As described in Section~\ref{sec:debiasing}, using the label-free metric helps lessen the influence of noisy labels. Therefore, we compute the entropy of each sample $x$ in epoch $e$ as follows:
\begin{equation}
    \label{eq:weight}
        \mc{H}_\tau(x,e)  = -\sum_{c}^C f_b(x,\tau)[c] \times \log f_b(x,\tau)[c], 
\end{equation}
Note that this score is independent of the given label $y_\text{given}$. Since, as training progresses, DNNs quickly memorize difficult-to-learn examples~\cite{liu2020early}, the ability to distinguish between bias-conflicting samples and bias-aligned samples is limited. We prevent this mixing effect by averaging $\mc{H}_\tau(x,e)$ over epochs~\cite{pleiss2020identifying}:
\begin{equation}
    \label{eq:ent_margin}
    \mc{E}(x)  = \frac{1}{E} \sum_{e=1}^E \mc{H}_\tau(x,e), 
\end{equation}
where $E$ denotes training epochs. We call the score $\mc{E}(x)$ the \emph{Entropy-margin} score.
Based on the calculated weight~\eqref{eq:ent_margin}, we give the probability of batch sampling for each sample as follows:
\begin{equation}
    \label{eq:sampling_prob}
    \mc{P}(x) = \frac{\mc{E}(x)}{\sum_{x} \mc{E}(x)}
\end{equation}

\myparagraph{Denoising after debiasing.}
As the final stage of \alg, perform denoising using batch $B$ generated by sampling with probability $\mc{P}(x)$. Note that any denoising algorithm is applicable. The availability of the denoising procedure is due to the fact that the biased dataset is balanced owing to the entropy-based weighted sample. Additionally, it allows the bias-conflicting samples to be learned with sufficient confidence. 

